Test-Time Domain Generalization via Universe Learning: A Multi-Graph Matching Approach for Medical Image Segmentation

Despite domain generalization (DG) has significantly addressed the performance degradation of pre-trained models caused by domain shifts, it often falls short in real-world deployment. Test-time adaptation (TTA), which adjusts a learned model using unlabeled test data, presents a promising solution. However, most existing TTA methods struggle to deliver strong performance in medical image segmentation, primarily because they overlook the crucial prior knowledge inherent to medical images. To address this challenge, we incorporate morphological information and propose a framework based on multi-graph matching. Specifically, we introduce learnable universe embeddings that integrate morphological priors during multi-source training, along with novel unsupervised test-time paradigms for domain adaptation. This approach guarantees cycle-consistency in multi-matching while enabling the model to more effectively capture the invariant priors of unseen data, significantly mitigating the effects of domain shifts. Extensive experiments demonstrate that our method outperforms other state-of-the-art approaches on two medical image segmentation benchmarks for both multi-source and single-source domain generalization tasks. The source code is available at https://github.com/Yore0/TTDG-MGM.

==> tables/re_prostate.tex <==
\begin{tabular}{c|cccccc|cc|ccc|c}
\hlineB{3}
\multirow{2}{*}{Methods} & \multicolumn{2}{c}{BMC} & \multicolumn{2}{c}{I2CVB} & \multicolumn{2}{c|}{HK} & \multicolumn{2}{c|}{Avg.} & \multicolumn{3}{c|}{Source Model Training} & \multicolumn{1}{c}{Inference}  \\ \cline{2-13} 
                         & \textit{DSC}      &  HD95    & \textit{DSC}      &  HD95& \textit{DSC}      &  HD95& \textit{DSC} $\uparrow$     &  HD95 $\downarrow$ &Params (M) $\downarrow$  &GFLops $\downarrow$ & Times$\downarrow$ (s) & Times$\downarrow$ (s/img) \\ \hline \hline

\textit{No Adapt} & 74.30 & 16.08 & 66.47 & 37.16 & 80.51 & 8.79 & 73.76 & 20.67 & \textbf{22.55} & \textbf{12.72} & 1.13 & \textbf{0.22} \\  \hline

TASD [8]& 76.28 & 15.11 & 68.30 & 31.43 & 81.09 & 4.26 & 75.22 & 16.93 & 40.88 & 20.35 & 1.63 & 0.37\\

VPTTA [3]& 77.42 & 12.93 & 70.25 & 30.01 & 83.27 & 3.40 & 76.98 & 15.45 &23.10 & 13.89 & \textbf{1.12} & 0.23 \\

PASS [79] & \textbf{80.07} & 10.50 &71.41 & 28.26 & 84.88 & 3.03 & 78.79 & 13.93 & 24.52 & 15.23 & 1.20 & 0.29 \\

Ours & 79.63 & \textbf{9.99} & \textbf{74.09} & \textbf{25.70} & \textbf{86.12} & \textbf{2.84} & \textbf{79.95} & \textbf{12.84} & 28.41 & 25.76 & 2.08 & 0.39 \\



\hlineB{3}
\end{tabular}

